DREAM: Debugging and Repairing AutoML Pipelines

Deep Learning models have become an integrated component of modern software systems. In response to the challenge of model design, researchers proposed Automated Machine Learning (AutoML) systems, which automatically search for model architecture and hyperparameters for a given task. Like other software systems, existing AutoML systems suffer from bugs. We identify two common and severe bugs in AutoML, performance bug (i.e., searching for the desired model takes an unreasonably long time) and ineffective search bug (i.e., AutoML systems are not able to find an accurate enough model). After analyzing the workflow of AutoML, we observe that existing AutoML systems overlook potential opportunities in search space, search method, and search feedback, which results in performance and ineffective search bugs. Based on our analysis, we design and implement DREAM, an automatic debugging and repairing system for AutoML systems. It monitors the process of AutoML to collect detailed feedback and automatically repairs bugs by expanding search space and leveraging a feedback-driven search strategy. Our evaluation results show that DREAM can effectively and efficiently repair AutoML bugs.

==> src/ack.tex <==
%!TEX root = ../main.tex

==> src/beam.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.9\columnwidth]{./figure/BeamVsGreedy1.pdf}
	\caption{Beam Search VS Greedy Search}\label{fig:beamvsgreedy}
	% \vspace{-15pt}
\end{figure}

\subsubsection{Another Strategy}
%  Alternative Strategy
\label{sec:alternative_search}


The feedback-driven search in \sys is an improved greedy search strategy.
Specifically, when searching for a new model, it picks the best performing model in the search history and modifies this model by selecting actions that are most likely to improve the model through the feedback-driven search, as shown from Line~\ref{line:initial} to Line~\ref{line:newmodel} in~\autoref{algo:overview}.

In fact, beam search, which is a common heuristic greedy search strategy, can be an alternative search method in \sys.
It builds the search tree with a breadth-first search over the search space and generates all successors of the states at each level of the tree and sorts them with their performance~\cite{beamsearch}.
The number of the stored states is equal to the width of the beam, which means that the larger the beam width, the fewer states to prune and the higher the search overhead.
When the beam width is 1, the search process will be equivalent to the greedy search.
With the above properties, beam search can explore the search space by expanding the most promising results in a limited set and is widely used in NLP and speech recognition models to choose the best output~\cite{stahlberg2019nmt,meister2020best}.

To determine the actual effect of beam search as an alternative search method, we construct a comparative experiment on the CIFAR-100 dataset.  The experiment ensures that the search priority and search space of the two search strategies are consistent.
In order to control the overhead of beam search, the beam width is set to 3.
In addition, with the intention of improving the search efficiency of beam search and covering more possible models in search, we implement a two-step search.
In the first step, we train nine searched models with the highest priorities, which are generated from the previous search, on a 10\% subset of the CIFAR-100 dataset.
Then in the second step, three models with the best performance in the first step are reserved for the complete training.
% Unlike greedy search, there are multiple models that can be searched for each search trial in beam search.
% Therefore, we use the sum of the model accuracy and the weight of the priority of feasible actions of this model to express the comprehensive priority of a specific model with a specific action.
% That is, the higher the expected performance of the model with the selected actions, the higher their search priority. 
In addition, in order to avoid beam search converging in local optimum, all hyperparameters in the models in searches have a chance of 0.01 to randomly mutate.

\autoref{fig:beamvsgreedy} shows the comparison results of beam search and greedy search on the CIFAR-100 dataset, where the X-axis is the GPU hours spent in the search, and the Y-axis is the best validation accuracy the search reached.
We implement two kinds of beam search in the experiments, namely a search trained in two steps with a 10\% subset of the dataset as described above (i.e., `Beam Search (Subset)'), and a search trained directly on the full dataset without the subset (i.e., `Beam Search (Full Dataset)'). 
The experimental results demonstrate the superiority of greedy search in search efficiency and effectiveness.
From~\autoref{fig:beamvsgreedy}, greedy search improves accuracy faster than beam search using subsets.
And beam search trained on the full dataset performs worst in these search methods.
We analyze the specific process of the search manually and find that the main reason for the performance difference is that the beam search trains more models, and most of them help little in improving the search performance.
This results in that the search efficiency of beam search is worse than that of greedy search in the case of the same search space and search priorities.
Even for the search that most of the models are training on the subset, the time spent of beam search to reach 80\% accuracy is still nearly 6 hours higher than the time spent of greedy search due to the time overhead of training additional models.

Therefore, for the consideration of efficiency and effectiveness in search, we select the greedy method as the default strategy of the feedback-driven search.
% fix the ineffective search and performance bugs more effectively.
We believe that beam search has the potential to achieve better results when computing resources are sufficient and training can be deployed in parallel.
% Therefore, a demo version of the beam search is implemented in \sys, as shown in our repository~\cite{ourrepo}. 
% We also implement the beam search strategy with priority, which is shown in our repository~\cite{ourrepo}.
It will be our future work to improve the effectiveness of the feedback-driven beam search. 

==> src/discussion.tex <==
%!TEX root = ../main.tex

==> src/effective_table.tex <==
% \begin{table*}[]
%     \centering
%     \scriptsize
%     \caption{Overall Results of 4 Search Methods with 25 Trials on 4 Datasets
%     \colorbox{red}{Effective table}}
%     \label{t:effective_result}
%     \tabcolsep=6pt
%     \begin{tabular}{crrrrrrrrrrrrrrrrrr}
%     \toprule
%     \multirow{2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{2}{*}{Num}} &
%     \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\
%     Score(\%)\end{tabular}}} & \multicolumn{4}{c}{Best Score(\%)} &
%     \multicolumn{4}{c}{Score Improvement(\%)} & \multicolumn{4}{c}{Improvement
%     Ratio} & \multicolumn{4}{c}{Trials to Reach Best Score} 
%     \\ 
%     \cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15}
%     \cmidrule(r){16-19}
%     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{AKG} &
%     \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
%     \multicolumn{1}{c}{\sys} & \multicolumn{1}{c}{AKG} &
%     \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
%     \multicolumn{1}{c}{\sys} & \multicolumn{1}{c}{AKG} &
%     \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
%     \multicolumn{1}{c}{\sys} & \multicolumn{1}{c}{AKG} &
%     \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
%     \multicolumn{1}{c}{\sys} \\
%     \midrule
%     \multirow{4}{*}{CIFAR-100} & 1 & 10.59 & 63.04 & \multicolumn{1}{l}{-} &
%     78.78 & 83.32 & 52.45 & \multicolumn{1}{l}{-} & 68.19 & 72.72 &
%     5.95 & \multicolumn{1}{l}{-} & 7.44 & 7.86 & 18 & \multicolumn{1}{l}{-} & 17
%     & 12 \\
%     & 2 & 22.77 & 34.23 & 67.79 & \multicolumn{1}{l}{-} & 82.66 &
%     11.46 & 45.01 & \multicolumn{1}{l}{-} & 59.89 & 1.50 & 2.98 &
%     \multicolumn{1}{l}{-} & 3.63 & 8 & 13 & \multicolumn{1}{l}{-} & 16 \\
%     & 3 & 22.33 & 37.63 & \multicolumn{1}{l}{-} & \multicolumn{1}{l}{-} &
%     82.62 & 15.30 & \multicolumn{1}{l}{-} & \multicolumn{1}{l}{-} & 60.29
%     & 1.69 & \multicolumn{1}{l}{-} & \multicolumn{1}{l}{-} & 3.70 & 25 &
%     \multicolumn{1}{l}{-} & \multicolumn{1}{l}{-} & 11 \\
%     & Ave & 18.57 & 44.97 & 67.79 & 78.78 & 82.87 & 26.40 & 45.01
%     & 68.19 & 64.30 & 2.42 & 3.65 & 4.24 & 4.46 & 17 & 13 & 17 & 13 \\ \midrule
%     \multirow{4}{*}{Food-101} & 4 & 8.37 & 72.67 & 57.47 & 51.59 &
%     83.13 & 64.31 & 49.10 & 43.22 & 74.77 & 8.69 & 6.87 & 6.17 & 9.94
%     & 25 & 1 & 15 & 23 \\
%     & 5 & 2.30 & 61.44 & 41.37 & 50.16 & 78.23 & 59.14 & 39.07 &
%     47.86 & 75.93 & 26.68 & 17.96 & 21.78 & 33.97 & 24 & 21 & 17 & 16 \\
%     & 6 & 8.48 & 68.80 & 75.72 & 55.61 & 82.62 & 60.32 & 67.25 &
%     47.13 & 74.14 & 8.12 & 8.93 & 6.56 & 9.75 & 25 & 13 & 20 & 19 \\
%     & Ave & 6.38 & 67.64 & 58.19 & 52.45 & 81.33 & 61.26 & 51.80 &
%     46.07 & 74.95 & 10.60 & 9.12 & 8.22 & 12.74 & 25 & 12 & 17 & 19 \\ \midrule
%     \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Stanford\\ Cars\end{tabular}} & 7
%     & 0.74 & 24.75 & 79.64 & 48.33 & 85.02 & 24.01 & 78.90 &
%     47.59 & 84.28 & 33.33 & 107.25 & 65.08 & 114.50 & 19 & 18 & 24 & 23 \\
%     & 8 & 0.56 & 42.70 & 81.99 & 24.44 & 83.66 & 42.14 & 81.44 &
%     23.89 & 83.11 & 76.67 & 147.22 & 43.89 & 150.22 & 24 & 21 & 9 & 19 \\
%     & 9 & 0.80 & 60.33 & 16.40 & 20.17 & 83.48 & 59.53 & 15.59 &
%     19.37 & 82.67 & 75.00 & 20.38 & 25.08 & 103.77 & 24 & 8 & 5 & 25 \\
%     & Ave & 0.70 & 42.59 & 59.34 & 30.98 & 84.06 & 41.89 & 58.64 &
%     30.28 & 83.35 & 60.73 & 84.62 & 44.18 & 119.85 & 22 & 16 & 13 & 22 \\ \midrule
%     \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} &
%     10 & 18.89 & 29.34 & 21.57 & 71.51 & 83.80 & 10.45 & 2.68 &
%     52.62 & 64.92 & 1.55 & 1.14 & 3.79 & 4.44 & 22 & 0 & 14 & 9 \\
%     & 11 & 9.44 & 62.86 & 42.29 & 44.70 & 79.90 & 53.43 & 32.86 &
%     35.27 & 70.46 & 6.66 & 4.48 & 4.74 & 8.47 & 21 & 5 & 24 & 23 \\
%     & 12 & 4.84 & 47.44 & 66.39 & 61.04 & 83.95 & 42.60 & 61.56 &
%     56.20 & 79.12 & 9.81 & 13.73 & 12.62 & 17.36 & 25 & 19 & 5 & 15 \\
%     & Ave & 11.05 & 46.54 & 43.42 & 59.08 & 82.55 & 35.49 & 32.36
%     & 48.03 & 71.50 & 4.21 & 3.93 & 5.35 & 7.47 & 23 & 8 & 14 & 16 \\ \midrule
%     \multicolumn{2}{c}{Ave} & 9.18 & 50.44 & 55.06 & 50.63 & 82.70 &
%     41.26 & 47.34 & 44.13 & 73.52 & 5.50 & 6.00 & 5.52 & 9.01 & 39 & 22
%     & 12 & 15 \\ \bottomrule
%     \end{tabular}
% \end{table*}


\begin{table*}[]
    \centering
    \scriptsize
    \caption{Overall Results of 4 Search Methods with 25 Trials on 4 Datasets}
    \label{t:effective_result}
    \tabcolsep=6pt
    \begin{tabular}{crrrrrrrrrrrrrrrrrr}
    \toprule
    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Best
    Score (\%)} & \multicolumn{4}{c}{Score Improvement (\%)} &
    \multicolumn{4}{c}{Improvement Ratio} & \multicolumn{4}{c}{Trials to Reach
    Best Score} \\ \cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15}
    \cmidrule(r){16-19}
    \multirow{-2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{-2}{*}{No.}} &
    \multicolumn{1}{c}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\
    Score (\%)\end{tabular}}} & \multicolumn{1}{c}{AKG} & \multicolumn{1}{c}{AKB}
    & \multicolumn{1}{c}{AKH} & \multicolumn{1}{c}{\sys} &
    \multicolumn{1}{c}{AKG} & \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH}
    & \multicolumn{1}{c}{\sys} & \multicolumn{1}{c}{AKG} &
    \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
    \multicolumn{1}{c}{\sys} & \multicolumn{1}{c}{AKG} &
    \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
    \multicolumn{1}{c}{\sys} \\ \midrule
    & 1 & 10.59 & 63.04 & 65.77 & 78.78 &
    \cellcolor{blue!20}83.32 & 52.45 & 55.18 & 68.19 &
    \cellcolor{blue!20}72.72 & 5.95 & 6.21 & 7.44 &
    \cellcolor{blue!20}7.86 & 18 & 25 & 17 & \cellcolor{blue!20}12 \\
    & 2 & 2.58 & 34.23 & 67.79 & 68.21 & \cellcolor{blue!20}82.66
    & 31.65 & 65.21 & 65.63 & \cellcolor{blue!20}80.09 & 13.28 &
    26.29 & 26.46 & \cellcolor{blue!20}32.06 & \cellcolor{blue!20}8 &
    13 & 22 & 16 \\
    & 3 & 8.19 & 37.63 & 64.49 & 73.15 & \cellcolor{blue!20}82.62
    & 29.44 & 56.30 & 64.97 & \cellcolor{blue!20}74.44 & 4.60 &
    7.88 & 8.94 & \cellcolor{blue!20}10.09 & 25 & 25 & 20 &
    \cellcolor{blue!20}11 \\
   \multirow{-4}{*}{CIFAR-100} & Ave & 7.12 & 44.97 & 66.01 & 73.38 &
     \cellcolor{blue!20}82.87 & 37.85 & 58.90 & 66.26 &
     \cellcolor{blue!20}75.75 & 6.32 & 9.27 & 10.31 &
     \cellcolor{blue!20}11.64 & 17.00 & 21.00 & 19.67 & \cellcolor{blue!20}13.00
     \\ \midrule
     & 4 & 8.37 & 72.67 & 57.47 & 51.59 &
     \cellcolor{blue!20}83.13 & 64.31 & 49.10 & 43.22 &
     \cellcolor{blue!20}74.77 & 8.69 & 6.87 & 6.17 &
     \cellcolor{blue!20}9.94 & 25 & \cellcolor{blue!20}1 & 15 & 23 \\
     & 5 & 2.30 & 61.44 & 41.37 & 50.16 &
     \cellcolor{blue!20}78.23 & 59.14 & 39.07 & 47.86 &
     \cellcolor{blue!20}75.93 & 26.68 & 17.96 & 21.78 &
     \cellcolor{blue!20}33.97 & 24 & 21 & 17 & \cellcolor{blue!20}16
     \\
     & 6 & 8.48 & 68.80 & 75.72 & 55.61 &
     \cellcolor{blue!20}82.62 & 60.32 & 67.25 & 47.13 &
     \cellcolor{blue!20}74.14 & 8.12 & 8.93 & 6.56 &
     \cellcolor{blue!20}9.75 & 25 & \cellcolor{blue!20}13 & 20 & 19 \\
    \multirow{-4}{*}{Food-101} & Ave & 6.38 & 67.64 & 58.19 & 52.45 &
    \cellcolor{blue!20}81.33 & 61.26 & 51.80 & 46.07 &
    \cellcolor{blue!20}74.95 & 10.60 & 9.12 & 8.22 &
    \cellcolor{blue!20}12.74 & 24.67 & \cellcolor{blue!20}11.67 & 17.33 & 19.33 \\ \midrule
     & 7 & 0.74 & 24.75 & 79.64 & 48.33 &
     \cellcolor{blue!20}85.02 & 24.01 & 78.90 & 47.59 &
     \cellcolor{blue!20}84.28 & 33.33 & 107.25 & 65.08 &
     \cellcolor{blue!20}114.50 & 19 & \cellcolor{blue!20}18 & 24 & 23 \\
     & 8 & 0.56 & 42.70 & 81.99 & 24.44 &
     \cellcolor{blue!20}83.66 & 42.14 & 81.44 & 23.89 &
     \cellcolor{blue!20}83.11 & 76.67 & 147.22 & 43.89 &
     \cellcolor{blue!20}150.22 & 24 & 21 & \cellcolor{blue!20}9 & 19
     \\
     & 9 & 0.80 & 60.33 & 16.40 & 20.17 &
     \cellcolor{blue!20}83.48 & 59.53 & 15.59 & 19.37 &
     \cellcolor{blue!20}82.67 & 75.00 & 20.38 & 25.08 &
     \cellcolor{blue!20}103.77 & 24 & 8 & \cellcolor{blue!20}5 & 25 \\
    \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Stanford\\ Cars\end{tabular}} & Ave & 0.70 & 42.59 & 59.34 & 30.98
    & \cellcolor{blue!20}84.06 & 41.89 & 58.64 & 30.28 &
    \cellcolor{blue!20}83.35 & 60.73 & 84.62 & 44.18 &
    \cellcolor{blue!20}119.85 & 22.33 & 15.67 & \cellcolor{blue!20}12.67 & 22.33
    \\ \midrule
     & 10 & 21.57 & 29.34 & 21.57 & 71.51 &
     \cellcolor{blue!20}83.80 & 10.45 & 2.68 & 52.62 &
     \cellcolor{blue!20}64.92 & 1.55 & 1.14 & 3.79 &
     \cellcolor{blue!20}4.44 & 22 & \cellcolor{blue!20}0 & 14 &
     \cellcolor{blue!20}9 \\
     & 11 & 9.44 & 62.86 & 42.29 & 44.70 &
     \cellcolor{blue!20}79.90 & 53.43 & 32.86 & 35.27 &
     \cellcolor{blue!20}70.46 & 6.66 & 4.48 & 4.74 &
     \cellcolor{blue!20}8.47 & 21 & \cellcolor{blue!20}5 & 24 & 23 \\
     & 12 & 4.84 & 47.44 & 66.39 & 61.04 &
     \cellcolor{blue!20}83.95 & 42.60 & 61.56 & 56.20 &
     \cellcolor{blue!20}79.12 & 9.81 & 13.73 & 12.62 &
     \cellcolor{blue!20}17.36 & 25 & 19 & \cellcolor{blue!20}5 & 15 \\
    \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} & Ave & 11.05 & 46.54 & 43.42 &
    59.08 & \cellcolor{blue!20}82.55 & 35.49 & 32.36 & 48.03 &
    \cellcolor{blue!20}71.50 & 4.21 & 3.93 & 5.35 &
    \cellcolor{blue!20}7.47 & 22.67 & \cellcolor{blue!20}8.00 & 14.33 & 15.67 \\ \midrule 
    \multicolumn{2}{c}{Ave} & 6.54 & 50.44 & 56.74 & 53.97 &
    \cellcolor{blue!20}82.70 & 44.12 & 50.43 & 47.66 &
    \cellcolor{blue!20}76.39 & 7.72 & 8.68 & 8.26 &
    \cellcolor{blue!20}12.65 & 41.87 & 21.67 & \cellcolor{blue!20}14.08 & 16.00 \\
    \bottomrule
    \end{tabular}
\end{table*}

==> src/efficiency_table.tex <==
% \begin{table}[]
%     \centering
%     \scriptsize
%     \caption{Overall Results of 4 Search Methods to Reach Target Accuracy on 4 Datasets}
%     % \xy{random search seems have more than expected performance... better than us and better than greedy(default of AK)}
%     \label{t:efficiency_result}
%     \tabcolsep=2.5pt
%     \begin{tabular}{crrrrrrrrrrr}
%       \toprule
%       \multirow{2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{2}{*}{Num}} &
%       \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\
%       Score (\%)\end{tabular}}} &
%       \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\
%       Score (\%)\end{tabular}}} & \multicolumn{4}{c}{Time to Reach Target (s)} &
%       \multicolumn{4}{c}{Best Score in 24 Hours(\%)} \\ \cmidrule(r){5-8} \cmidrule(r){9-12}
%       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &
%       \multicolumn{1}{c}{AKG} & \multicolumn{1}{c}{AKB} &
%       \multicolumn{1}{c}{AKH} & \multicolumn{1}{c}{\sys} &
%       \multicolumn{1}{c}{AKG} & \multicolumn{1}{c}{AKB} &
%       \multicolumn{1}{c}{AKH} & \multicolumn{1}{c}{\sys} \\ \midrule
%       \multirow{3}{*}{CIFAR-100} & 1 & 10.59 & 70 & - & - & 1.63 & 0.92 &
%       63.04 & 52.51 & 79.19 & 83.32 \\
%       & 2 & 2.58 & 70 & 18.32 & - & 5.45 & 1.80 & 77.79 & 67.79 &
%       80.21 & 82.66 \\
%       & 3 & 8.19 & 70 & - & 17.97 & 1.36 & 0.53 & 42.57 & 76.52 &
%       78.89 & 82.62 \\ \midrule
%       \multirow{3}{*}{Food-101} & 4 & 8.37 & 70 & 40.35 & - & - & 21.66 &
%       61.68 & 57.47 & 59.42 & 77.23 \\
%       & 5 & 2.30 & 70 & - & - & - & 45.04 & 13.57 & 31.93 & 58.74 &
%       65.74 \\
%       & 6 & 8.48 & 70 & - & 82.24 & - & 13.34 & 13.54 & 60.43 & 55.61
%       & 72.26 \\ \midrule
%       \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Stanford\\ Cars\end{tabular}} &
%       7 & 0.74 & 70 & - & 9.48 & - & 4.03 & 30.75 & 78.22 & 55.57 &
%       83.79 \\
%       & 8 & 0.56 & 70 & 16.87 & 8.38 & - & 7.85 & 71.53 & 81.99 &
%       46.66 & 83.35 \\
%       & 9 & 0.80 & 70 & - & - & - & 17.57 & 7.61 & 16.40 & 40.72 &
%       70.61 \\ \midrule
%       \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} &
%       10 & 18.89 & 70 & - & - & 1.71 & 2.60 & 27.38 & 21.57 & 76.97 &
%       83.80 \\
%       & 11 & 9.44 & 70 & - & - & 4.17 & 2.85 & 62.78 & 42.29 & 80.26 &
%       77.93 \\
%       & 12 & 4.83 & 70 & - & - & 10.00 & 2.54 & 42.13 & 41.70 & 80.09
%       & 77.02 \\ \bottomrule
%      \end{tabular}
% \end{table}

\begin{table}[]
  \centering
  \scriptsize
  \caption{Overall Results of 4 Search Methods to Reach Target Accuracy on 4 Datasets}
  % \xy{random search seems have more than expected performance... better than us and better than greedy(default of AK)}
  \label{t:efficiency_result}
  \tabcolsep=3pt
  \begin{tabular}{crrrrrrrrrr}
    \toprule
    \multirow{2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{2}{*}{No.}} &
    \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\
    Score (\%)\end{tabular}}} & \multicolumn{4}{c}{Time to Reach 70
    Accuracy (h)} & \multicolumn{4}{c}{Best Score in 24 Hours (\%)} \\ \cmidrule(r){4-7} \cmidrule(r){8-11}
    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{AKG} &
    \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
    \multicolumn{1}{c}{\textbackslash{}sys} & \multicolumn{1}{c}{AKG} &
    \multicolumn{1}{c}{AKB} & \multicolumn{1}{c}{AKH} &
    \multicolumn{1}{c}{\textbackslash{}sys} \\ \midrule
    \multirow{3}{*}{CIFAR-100} & 1 & 10.59 & - & - & 1.63 & 0.92 & 63.04 &
    52.51 & 79.19 & 83.32 \\
    & 2 & 2.58 & 18.32 & - & 5.45 & 1.80 & 77.79 & 67.79 & 80.21 &
    82.66 \\
    & 3 & 8.19 & - & 17.97 & 1.36 & 0.53 & 42.57 & 76.52 & 78.89 &
    82.62 \\ \midrule
    \multirow{3}{*}{Food-101} & 4 & 8.37 & 40.35 & - & - & 21.66 & 61.68 &
    57.47 & 59.42 & 71.56 \\
    & 5 & 2.30 & - & - & - & 45.04 & 13.57 & 31.93 & 58.74 & 65.74 \\
    & 6 & 8.48 & - & 82.24 & - & 13.34 & 13.54 & 35.94 & 55.61 & 72.03
    \\ \midrule
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Stanford\\ Cars\end{tabular}} & 7
    & 0.74 & - & 9.48 & - & 4.03 & 30.76 & 77.60 & 55.57 & 83.79 \\
    & 8 & 0.56 & 16.87 & 8.38 & - & 7.85 & 71.53 & 81.99 & 46.66 &
    83.35 \\ 
    & 9 & 0.80 & - & - & - & 17.57 & 7.61 & 16.40 & 40.72 & 70.61 \\ \midrule
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Tiny\\ ImageNet\end{tabular}} &
    10 & 18.89 & - & - & 1.71 & 2.60 & 27.38 & 21.57 & 76.98 & 77.67
    \\
    & 11 & 9.44 & - & - & 4.17 & 2.85 & 62.78 & 42.29 & 80.26 & 76.66
    \\
    & 12 & 4.83 & - & - & 10.00 & 2.54 & 42.13 & 41.70 & 80.09 & 77.02 \\
    \bottomrule
   \end{tabular}
\end{table}


==> src/related.tex <==
%!TEX root = ../main.tex
\section{Related Work}
\label{sec:related}

DL techniques are widely used to benefit in various SE
tasks~\cite{madala2017automated,joulin2015inferring,tong2018software,pang2017predicting,dahl2013large,hellendoorn2017deep,dwivedi2016software}.
In this paper, we debug the efficiency and effectiveness problems in the
existing AutoML pipelines.
To solve these problems, we propose and implement \sys which consists of two
repair modules, search space expansion and priority-based search.
It is highly related with automated machine learning and DL system debugging.
%  and automatic program repair.

\smallskip
\noindent
{\bf Automated Machine Learning}
Automated Machine Learning (AutoML) focuses on automatically design models for given training tasks.  In the
early stage of AutoML, the works usually focus on traditional machine learning,
and various tools are designed to be applied in various scenarios such as
Auto-WEKA~\cite{thornton2013auto}, TPOT~\cite{olson2016tpot},
hyperopt-sklearn~\cite{komer2019hyperopt} and
autosklearn~\cite{AutoSklearn,feurer2019auto,feurer2020auto}.
Their optimization methods mainly contains Bayesian optimization, evolutionary
algorithms~\cite{brochu2010tutorial,shahriari2015taking,feurer2019hyperparameter}.
% These tools can choose the suitable ML algorithms and corresponding
% hyperparameters by these optimization methods to solve
% the combined algorithm selection and hyperparameter (CASH) problem.
% Therefore, the models they generate can often perform well on the given tasks.
These works mainly focus on traditional machine learning pipeline while \sys
focuses on the repair and improvement on the search of DNN models. 

With the development of DNN, NAS and HPO algorithms that are good at determining
well-performing DNN architecture and tuning suitable hyperparameters for a given
dataset have become a new trend of search methods in AutoML. 
Common NAS algorithms include Bayesian
optimization~\cite{snoek2012practical,zela2018towards,kandasamy2018neural,negrinho2017deeparchitect,dikov2019bayesian,white2019bananas,jin2019auto},
deep reinforcement
learning~\cite{zoph2016neural,baker2016designing,pham2018efficient,zoph2018learning},
evolutionary
algorithms~\cite{guo2020single,real2017large,xie2017genetic,suganuma2017genetic},
and gradient based
methods~\cite{luo2018neural,cai2018proxylessnas,liu2018darts,wu2018mixed,dong2019searching,he2020milenas}.
And HPO algorithms mainly base on Bayesian Optimization
method~\cite{snoek2012practical,rasmussen2003gaussian,bergstra2011algorithms,bergstra2013hyperopt,hutter2011sequential},
gradient-based
method~\cite{pedregosa2016hyperparameter,maclaurin2015gradient,chandra2019gradient}.
% Although, the AutoML pipelines with these search methods have achieved outstanding results in searching
% architectures and hyperparameters on the
% various datasets, their searches often spend lots of time and search trials, and even may
% require hundreds of GPU days. \sys dedicates to search for a satisfactory neural
% architecture with as short as possible time and improve the search efficiency.
Based on the existing optimization methods on searching models, the open-source
AutoML pipelines for DNN are implemented, such as
AutoNet~\cite{mendoza2019towards},Auto-Pytorch~\cite{zimmer2021auto}, Microsoft
NNI~\cite{MicrosoftNNI}, and AutoKeras~\cite{AutoKeras}.
% These pipelines show outstanding search results in actual application.
The most popular among them are Microsoft NNI and AutoKeras.
NNI which is implemented on the DL framework Retiarii~\cite{zhang2020retiarii} prefers to provide
users with a complete AutoML toolkit, including neural
architecture search, hyperparameter tuning and model compression.
% Its expected users are practitioners with certain expertise.
AutoKeras is based on TensorFlow and implements 3 search algorithms (i.e.,
Greedy, Bayesian~\cite{jin2019auto}, Hyperband~\cite{li2017hyperband}) besides
Random search. 
It provides a simple operation interface and implements a highly
automated model search pipeline, making it easy for users without any professional
knowledge to use.
% However, because their search methods often consider the search process as a ML
% problem, their searches often requires lots of time and search trials to fit the
% ML model to solve the problem, and even may require several GPU days.
However, these pipelines are still facing problems of search efficiency and search
effectiveness, which limit their practical use.
In this paper, we choose AutoKeras as the object for debugging and repairing
because it provides a highly automated model search pipeline and an easy-to-use
interface. 
\sys currently repairs the efficiency and effectiveness problems of the AutoKeras
pipelines, and the solutions in \sys is also theoretically applicable to other
AutoML pipelines.
% How to repair the problems in other AutoML pipelines will be one of our future directions. 
How to generalize and implement the repair method of \sys in other pipelines
will be one of our future directions. 
% \sys repairs the search efficiency
% and effectiveness problems with the search space expansion module and
% priority-based search module.
% It   And we implement our system based on AutoKeras and compare
% with three search methods in it.

% \smallskip
% \noindent
% {\bf Software Debugging.}



\smallskip
\noindent
{\bf Automatic Program Repair.}
Automatic program repair is designed to find bugs in programs and automatically
generate patches to fix them. Its process mainly includes fault location, patch
candidates generation and patch candidates validation. 
In order to repair programs efficiently, existing research on automated program
repair applies different patch generation methods, such as search-based
generation
methods~\cite{arcuri2008novel,weimer2009automatically,weimer2010automatic},
brute-force-based generation
methods~\cite{dallmeier2009generating,weimer2013leveraging,qi2015analysis},
semantic-based patch construction methods~\cite{jha2010oracle,nguyen2013semfix,hua2018towards}, etc. 
More program repair work can be found in the survey~\cite{gazzola2017automatic}.
Different from these research efforts, our work is to fix the efficiency and
effectiveness problems of the AutoML pipeline. These problems will not directly lead to program
crash like common bugs. And they can not be fixed by directly generating patches,
but rather through applying the specific solutions and restarting the search process. 


==> tftex/design_figure.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./figure/design_demo.pdf} 
	\caption{The Priority Guides the Search for Actions to Improve the Model Performance}\label{fig:designdemo}
	% \vspace{-15pt}
\end{figure}



==> tftex/priority_table.tex <==
\begin{table*}[]
    \caption{Partial Search Priority of Actions}
    % \xy{Draw a new table}
    \label{tab:priority}
    \centering
    \scriptsize
    \tabcolsep=3pt
    \begin{tabular}{lrrrrrr}
    \toprule
    % \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Conditions}}} &
    % \multicolumn{5}{c}{\textbf{Search Priority}} \\ \cmidrule{2-6}
    % \multicolumn{1}{c}{} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} &
    % \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{5} \\
    
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Conditions}}}  &
    \multicolumn{6}{c}{\textbf{Search Priority}}\\ \cmidrule{2-7}
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{1st} & \multicolumn{1}{c}{2nd} &
    \multicolumn{1}{c}{3rd} & \multicolumn{1}{c}{4th} & \multicolumn{1}{c}{5th}
    & \multicolumn{1}{c}{6th} \\
    \midrule
    EA-NC-DG-NW & trainable=True & imagenet size=True & block type=xception &
    optimizer=adam weight decay & optimizer=nadam & end learning rate=1e=5 \\
    EA-NC-EG-NW & trainable=True & block type=xception & imagenet size=True &
    version=b7 & optimizer=adam weight decay & end learning rate=1e=5 \\
    EA-NC-NG-NW & trainable=True & block type=xception & imagenet size=True &
    double step=True & dropout=0.5 & triple step=True \\
    EA-NC-VG-NW & trainable=True & imagenet size=True & block type=xception &
    momentum=0.1 & momentum=0.5 & learning rate=0.0001 \\
    EA-SC-DG-NW & trainable=True & imagenet size=True & block type=xception &
    momentum=0.1 & momentum=0.5 & learning rate=0.001 \\
    EA-SC-EG-NW & trainable=True & learning rate=0.01 & imagenet size=True &
    block type=xception & optimizer=adam & optimizer=adam weight decay \\
    RA-NC-EG-NW & block type=xception & trainable=True & imagenet size=True &
    augment=False & vertical flip=False & pretrained=False \\
    RA-NC-NG-NW & block type=xception & trainable=True & imagenet size=True &
    optimizer=adam weight decay & dropout=0.5 & end learning rate=1e=5 \\
    RA-SC-DG-NW & learning rate=0.0001 & trainable=True & learning rate=0.001 &
    block type=xception & learning rate=2e=05 & learning rate=1e=05 \\
    RA-SC-NG-NW & learning rate=0.01 & trainable=True & learning rate=0.1 &
    learning rate=0.001 & optimizer=adam weight decay & end learning rate=1e=5
    \\
    OA-NC-DG-NW & block type=xception & filters=256 & optimizer=adam weight
    decay & end learning rate=1e=5 & optimizer=nadam & learning rate=0.001 \\
    OA-NC-EG-EW & num blocks=1 & num layers=2 & optimizer=sgd & block
    type=xception & momentum=0.1 & separable=True \\
    OA-NC-NG-NW & block type=xception & separable=False & optimizer=adam weight
    decay & end learning rate=1e=5 & dropout=0.5 & optimizer=nadam \\
    OA-SC-DG-NW & block type=xception & learning rate=0.01 & learning rate=0.001
    & optimizer=sgd & momentum=0.1 & momentum=0.5 \\
    OA-SC-EG-EW & num blocks=3 & block type=xception & num layers=2 &
    separable=True & reduction type=global max & reduction type=global avg \\
    OA-SC-NG-NW & block type=xception & optimizer=adam weight decay & end
    learning rate=1e=5 & optimizer=nadam & learning rate=0.01 & learning
    rate=0.1 \\
    XA-NC-NG-NW & pretrained=True & trainable=True & imagenet size=True &
    optimizer=adam weight decay & dropout=0.5 & end learning rate=1e=5\\
    \bottomrule
    \end{tabular}
    \vspace{-10pt}
\end{table*}
